AllClear: A Comprehensive Dataset and Benchmark for Cloud Removal in Satellite Imagery

Clouds in satellite imagery pose a significant challenge for downstream applications. A major challenge in current cloud removal research is the absence of a comprehensive benchmark and a sufficiently large and diverse training dataset. To address this problem, we introduce the largest public dataset -- $\textit{AllClear}$ for cloud removal, featuring 23,742 globally distributed regions of interest (ROIs) with diverse land-use patterns, comprising 4 million images in total. Each ROI includes complete temporal captures from the year 2022, with (1) multi-spectral optical imagery from Sentinel-2 and Landsat 8/9, (2) synthetic aperture radar (SAR) imagery from Sentinel-1, and (3) auxiliary remote sensing products such as cloud masks and land cover maps. We validate the effectiveness of our dataset by benchmarking performance, demonstrating the scaling law -- the PSNR rises from $28.47$ to $33.87$ with $30\times$ more data, and conducting ablation studies on the temporal length and the importance of individual modalities. This dataset aims to provide comprehensive coverage of the Earth's surface and promote better cloud removal results.

==> defs.tex <==
\usepackage{color}

\newcommand{\xhdr}[1]{\vspace{-8pt} \paragraph*{{\bf #1}}}

\definecolor{ut_color_mark}{rgb}{0,0.5,1}
\definecolor{kb_color}{rgb}{0.2,.64,0}
\definecolor{question_color}{rgb}{0.0863, 0.149, 0.498}
\definecolor{black}{rgb}{0.0,0.0, 0.0}


\newcommand{\kb}[1]{\textsf{\textcolor{kb_color}{[{\bf KB says}: #1]}}}
\newcommand{\kbinline}[1]{\textsf{\textcolor{kb_color}{#1}}}
\newcommand{\kbmark}[1]{\textsf{\textcolor{kb_color_mark}{#1}}}
\newcommand{\ut}[1]{\textsf{\textcolor{ut_color_mark}{[{\bf UM}: #1]}}}
\newcommand{\bh}[1]{\textcolor{red}{BH: #1}}
\newcommand{\quest}[1]{\textcolor{question_color}{#1}}
\newcommand{\new}[1]{\textcolor{black}{#1}}

\newenvironment{packed_enum}{
\begin{enumerate}
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{2pt}
  \setlength{\parsep}{0pt}
}{\end{enumerate}}

\newenvironment{packed_item}{
\begin{itemize}
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{2pt}
  \setlength{\parsep}{0pt}
}{\end{itemize}}


==> deprecated/4_method.tex <==
\section{Method} % temporarily generated by GPT, need re-write.

\subsection{Problem formulation and setup}

% \begin{figure}
%   \centering
%   \includegraphics[width=\textwidth]{images/problem_setup.png}
%   \caption{Problem setup overview. For a given time period T, we assume Earth surface is unchanged. Given sparsely distributed MSI and SAR inputs, we generate one clear MSI for each day within the time period. The ground truth for evaluation is explained in the method section.}
%   \label{fig:problem_setup}
% \end{figure}
\cpp{multimodal and multi-temporal seems unnecessary. Maybe be just say we formulate the cloud removal task as a sequence-to-sequence task }
We formulate multimodal and multi-temporal cloud removal into a sequence-to-sequence framework, as depicted in Figure~\ref{fig:problem_setup}. For a predefined time period $T$, we treat the Earth's surface as static. Given every multi-spectral and SAR images during this time period as inputs, our task is to generate a clear multi-spectral output for each day within $T$. 

To mitigate the challenge of missing ground truth, we use Synthetic Cloud (SynCloud) to provide indirect supervision signals as used in \cite{zhao2023seeing}. The design is simple: for a given clear or partially clear mutli-spectral images, we randomly sample a cloud mask from the training set and merge them with the existing cloud masks. A reconstruction loss is computed in the regions under the additional cloud mask.

\subsection{Sequence-to-sequence model architecture}

% \begin{figure}
%   \centering
%   \includegraphics[width=\textwidth]{images/dae.png}
%   \caption{Model overview.}
%   \label{fig:dae}
% \end{figure}

The model architecture, illustrated in Figure~\ref{fig:model}, leverages a 3D-UNet design adapted from temporal sequence processing. This architecture facilitates the dense prediction necessary for translating multi-date, multi-modal inputs into a sequence of cloud-free images. Each layer of the network encodes features at different scales, with skip connections used to preserve spatial and temporal information across layers. The sequence-to-sequence nature of the model allows it to capture temporal dependencies and variations in cloud coverage, providing a coherent output sequence that closely mirrors the dynamics observed in satellite data.


\subsection{Denoising autoencoder training recipe}
Training of the denoising autoencoder was conducted on an NVIDIA A6000 GPU, focusing on robustness and generalization across diverse conditions. We utilized a combination of mean squared error (MSE) for pixel-level accuracy and a structural similarity index (SSIM) for maintaining textural integrity in the outputs. Data augmentation strategies, including synthetic cloud injection and varying levels of noise, were employed to enhance the model's ability to generalize from our extensive AllClear dataset. The model was trained using an Adam optimizer, and batch size was set to 4 to balance between computational efficiency and memory constraints.

\subsection{Latent Diffusion Model}
We plan to use the latent space of this denoising autoencoder (DAE) to train a latent diffusion model if the DAE cannot fully leverage the scale of \textit{AllClear}. But since the model is still in the training process, we reserve this part for future work.

==> tables/exp_allclear_dataset_full.tex <==
\begin{table}[th]
\caption{Benchmark Performance for models retrained on AllClear.}
\label{datasets}
\centering
\begin{footnotesize}
\begin{tabular}{l l c c c c c c c}
\toprule
\rowcolor{white}
Model 
& Evaluation Dataset 
& \multicolumn{1}{p{3cm}}{\centering Training Dataset \\ (fraction used)} 
& PSNR $(\uparrow)$ 
& SSIM $(\uparrow)$ 
& SAM $(\downarrow)$ 
& MAE $(\downarrow)$ \\
\midrule
\multirow{7}{*}{UnCRtainTS} 
& \multirow{5}{*}{\footnotesize{SEN12MS-CR-TS} } 
& SEN12MS-CR-TS
& \textbf{27.838}
& \textbf{0.866}
& \textbf{9.455}
& \textbf{0.036}
\\
& 
& \cellcolor{gray!25} AllClear ($1\%$)
& \cellcolor{gray!25} 24.242
& \cellcolor{gray!25} 0.796
& \cellcolor{gray!25} 13.379
& \cellcolor{gray!25} 0.049
\\
& 
& \cellcolor{gray!25} AllClear ($3.4\%$)
& \cellcolor{gray!25} 26.256
& \cellcolor{gray!25} 0.847
& \cellcolor{gray!25} 10.411
& \cellcolor{gray!25} 0.041
\\
& 
& \cellcolor{gray!25} AllClear ($10\%$)
& \cellcolor{gray!25} 27.570
& \cellcolor{gray!25} 0.852
& \cellcolor{gray!25} 10.758
& \cellcolor{gray!25} 0.038
\\
& 
& \cellcolor{gray!25} AllClear ($100\%$)
& \cellcolor{gray!25} 27.693
& \cellcolor{gray!25} 0.857
& \cellcolor{gray!25} 9.736
& \cellcolor{gray!25} 0.038
\\
\cline{2-7}
& \multirow{2}{*}{AllClear} 
& SEN12MS-CR-TS
& \textbf{29.009}
& 0.898
& \textbf{5.972}
& 0.039
\\
& 
& \cellcolor{gray!25} AllClear ($3.4\%$)
& \cellcolor{gray!25} 28.474 
& \cellcolor{gray!25} \textbf{0.906}
& \cellcolor{gray!25} 6.373
& \cellcolor{gray!25} \textbf{0.036}
\\
\bottomrule
\end{tabular}\label{table:benchmark_comparison}
\end{footnotesize}
\end{table}



\begin{table}[th]
\caption{Benchmark Performance for models retrained on AllClear.}
\label{datasets}
\centering
\begin{footnotesize}
\begin{tabular}{l l c c c c c c c}
\toprule
\rowcolor{white}
Model 
& Evaluation Dataset 
& \multicolumn{1}{p{3cm}}{\centering Training Dataset \\ (fraction used)} 
& PSNR $(\uparrow)$ 
& SSIM $(\uparrow)$ 
& SAM $(\downarrow)$ 
& MAE $(\downarrow)$ \\
\midrule
\multirow{7}{*}{UnCRtainTS} 
& \multirow{5}{*}{\footnotesize{SEN12MS-CR-TS} } 
& SEN12MS-CR-TS
& \textbf{27.838}
& \textbf{0.866}
& \textbf{9.455}
& \textbf{0.036}
\\
& 
& \cellcolor{gray!25} AllClear ($1\%$)
& \cellcolor{gray!25} 24.242
& \cellcolor{gray!25} 0.796
& \cellcolor{gray!25} 13.379
& \cellcolor{gray!25} 0.049
\\
& 
& \cellcolor{gray!25} AllClear ($3.4\%$)
& \cellcolor{gray!25} 26.256
& \cellcolor{gray!25} 0.847
& \cellcolor{gray!25} 10.411
& \cellcolor{gray!25} 0.041
\\
& 
& \cellcolor{gray!25} AllClear ($10\%$)
& \cellcolor{gray!25} 27.570
& \cellcolor{gray!25} 0.852
& \cellcolor{gray!25} 10.758
& \cellcolor{gray!25} 0.038
\\
& 
& \cellcolor{gray!25} AllClear ($100\%$)
& \cellcolor{gray!25} 27.693
& \cellcolor{gray!25} 0.857
& \cellcolor{gray!25} 9.736
& \cellcolor{gray!25} 0.038
\\
\cline{2-7}
& \multirow{2}{*}{AllClear} 
& SEN12MS-CR-TS
& \textbf{29.009}
& 0.898
& \textbf{5.972}
& 0.039
\\
& 
& \cellcolor{gray!25} AllClear ($3.4\%$)
& \cellcolor{gray!25} 28.474 
& \cellcolor{gray!25} \textbf{0.906}
& \cellcolor{gray!25} 6.373
& \cellcolor{gray!25} \textbf{0.036}
\\
\bottomrule
\end{tabular}\label{table:benchmark_comparison}
\end{footnotesize}
\end{table}




% \begin{table}[ht]
% \caption{Benchmark Performance for models retrained on AllClear.}
% \label{datasets}
% \centering
% \begin{footnotesize}
% \begin{tabular}{l l c c c c c c c}
% \toprule
% \rowcolor{white}
% Model & Evalation Dataset & Pretrain Dataset & PSNR $(\uparrow)$ & SSIM $(\uparrow)$ & SAM $(\downarrow)$ & MAE $(\downarrow)$ \\
% \midrule
% \multirow{7}{*}{UnCRtainTS} 
% & \multirow{5}{*}{SEN12MS-CR-TS } 
% & SEN12MS-CR-TS
% & \textbf{27.838}
% & \textbf{0.866}
% & \textbf{9.455}
% & \textbf{0.036}
% \\
% & 
% & \cellcolor{gray!25} AllClear ($1\%$)
% & \cellcolor{gray!25} 26.255
% & \cellcolor{gray!25} 0.847
% & \cellcolor{gray!25} 10.417
% & \cellcolor{gray!25} 0.041
% \\
% & 
% & AllClear ($3.4\%$)
% & 26.256
% & 0.847
% & 10.411
% & 0.041
% \\
% & 
% & \cellcolor{gray!25} AllClear ($10\%$)
% & \cellcolor{gray!25} 27.56
% & \cellcolor{gray!25} 0.852
% & \cellcolor{gray!25} 10.758
% & \cellcolor{gray!25} 0.038
% \\
% & 
% & AllClear ($100\%$)
% & 27.693
% & 0.857
% & 9.736
% & 0.038
% \\
% \cline{2-7}
% & \multirow{2}{*}{AllClear} 
% & SEN12MS-CR-TS
% & \textbf{29.009}
% & 0.898
% & \textbf{5.972}
% & 0.039
% \\
% & 
% & \cellcolor{gray!25} AllClear ($3.4\%$)
% & \cellcolor{gray!25} 28.474 
% & \cellcolor{gray!25} \textbf{0.906}
% & \cellcolor{gray!25} 6.373
% & \cellcolor{gray!25} \textbf{0.036}
% \\
% \bottomrule
% \end{tabular}\label{table:benchmark_comparison}
% \end{footnotesize}
% \end{table}





% \begin{table}[ht]
% \caption{Benchmark Performance for models retrained on AllClear.}
% \label{datasets}
% \centering
% \begin{footnotesize}
% \begin{tabular}{l l c c c c c c c}
% \toprule
% \rowcolor{white}
% Model & Eval. Dataset & Pretrain Dataset & PSNR $(\uparrow)$ & SSIM $(\uparrow)$ & SAM $(\downarrow)$ & MAE $(\downarrow)$ \\
% \midrule
% \multirow{4}{*}{UnCRtainTS} 
% & \multirow{2}{*}{SEN12MS-CR-TS } 
% & SEN12MS-CR-TS
% & \textbf{27.838}
% & \textbf{0.866}
% & \textbf{9.455}
% & \textbf{0.036}
% \\
% & 
% & \cellcolor{gray!25} AllClear
% &\cellcolor{gray!25} 26.255
% & \cellcolor{gray!25} 0.847
% & \cellcolor{gray!25} 10.417
% & \cellcolor{gray!25} 0.041
% \\
% \cline{3-7}
% & \multirow{2}{*}{AllClear} 
% & SEN12MS-CR-TS
% & \textbf{29.009}
% & 0.898
% & \textbf{5.972}
% & 0.039
% \\
% & 
% & \cellcolor{gray!25} AllClear
% & \cellcolor{gray!25} 28.474 
% & \cellcolor{gray!25} \textbf{0.906}
% & \cellcolor{gray!25} 6.373
% & \cellcolor{gray!25} \textbf{0.036}
% \\
% \bottomrule
% \end{tabular}\label{table:benchmark_comparison}
% \end{footnotesize}
% \end{table}

% \begin{table}[ht]
% \caption{Scaling law of our model on our AllClear datasets with UnCRtainTS as backbone architecture.}
% \label{datasets}
% \centering
% \begin{footnotesize}
% \begin{tabular}{l l c c c c c}
% \toprule
% \rowcolor{white}
% Fraction of Data & PSNR $(\uparrow)$ & SSIM $(\uparrow)$ & SAM $(\downarrow)$ & MAE $(\downarrow)$ \\
% \midrule
% 1\%
% & 29.009
% & 0.898
% & 5.972
% & 0.039
% \\
% 3.4\%
% & 28.474
% & 0.906
% & 6.373
% & 0.036
% \\
% 10\%
% & 32.997
% & 0.923
% & 6.038
% & \textbf{0.023}
% \\
% 100\%
% & \textbf{33.177}
% & \textbf{0.926}
% & \textbf{5.650}
% & \textbf{0.023}
% \\
% \bottomrule
% \end{tabular}
% \end{footnotesize}
% \end{table}

==> tables/exp_baseline.tex <==
\begin{table}[ht]
\caption{Benchmark performance of previous SoTA models evaluated on our AllClear benchmark dataset. The best performing values are in \textbf{bold} and the second best is \underline{underlined}.}
\label{datasets}
\centering
\begin{footnotesize}
\begin{tabular}{l l c c c c c c}
\toprule
\rowcolor{white}
Model & Training Dataset & PSNR $(\uparrow)$ & SSIM $(\uparrow)$ & SAM $(\downarrow)$ & MAE $(\downarrow)$ \\
\midrule
Least Cloudy
& \cellcolor{gray!25}-
& \cellcolor{gray!25} 28.864
& \cellcolor{gray!25} \underline{0.836}
& \cellcolor{gray!25} \underline{6.982}
& \cellcolor{gray!25} 0.078
\\
Mosaicing 
& -
& \textbf{29.824}
& 0.754
& 23.58
& \textbf{0.045}
\\
\midrule
UnCRtainTS~\citep{ebel2023uncrtaints} 
& \cellcolor{gray!25}SEN12MS-CR-TS 
& \cellcolor{gray!25} \underline{29.009}
& \cellcolor{gray!25}\textbf{0.898}
& \cellcolor{gray!25}\textbf{5.972}
& \cellcolor{gray!25} \underline{0.039}
\\
U-TILISE~\citep{stucker2023u} 
& SEN12MS-CR-TS 
& 24.660
& {0.807}
& {7.765}
& 0.083
\\
\bottomrule
\end{tabular}\label{table:benchmark_baselines}
\end{footnotesize}
\end{table}

==> tables/exp_baseline_all.tex <==
\begin{table}[ht]
\caption{Benchmark performance of previous SoTA models evaluated on our AllClear benchmark dataset. 
% The best performing values are in \textbf{bold}.
}
\label{datasets}
\centering
\begin{footnotesize}
\begin{tabular}{l l c c c c c c}
\toprule
\rowcolor{white}
Model & Training Dataset & PSNR $(\uparrow)$ & SSIM $(\uparrow)$ & SAM $(\downarrow)$ & MAE $(\downarrow)$ \\
\midrule
Least Cloudy
& -
& 28.864
& 0.836
& 6.982
& 0.078
\\
Mosaicing 
& -
& 29.824
& 0.754
& 23.58
& 0.045
\\
\midrule
UnCRtainTS
& SEN12MS-CR-TS 
& 29.009
& 0.898
& 5.972
& 0.039
\\
U-TILISE
& SEN12MS-CR-TS 
& 24.660
& 0.807
& 7.765
& 0.083
\\
CTGAN
& Sen2\_MTC
& 27.783
& 0.840
& 8.800
& 0.041
\\
PMAA
& STGAN
& 12.455
& 0.460
& 8.072
& 0.240
\\
PMAA
& Sen2\_MTC
& 24.328
& 0.768
& 8.680
& 0.078
\\
DiffCR
& STGAN
& 17.998
& 0.642
& 9.512
& 0.117
\\
DiffCR 
& Sen2\_MTC
& 25.220
& 0.744
& 9.382
& 0.060
\\
\bottomrule
\end{tabular}\label{table:benchmark_baselines_all}
\end{footnotesize}
\end{table}
